Are Heterogeneous Cloud-Based Radio Access Networks Cost Effective?

Mobile networks of the future are predicted to be much denser than today's networks in order to cater to increasing user demands. In this context, cloud based radio access networks have garnered significant interest as a cost effective solution to the problem of coping with denser networks and providing higher data rates. However, to the best knowledge of the authors, a quantitative analysis of the cost of such networks is yet to be undertaken. This paper develops a theoretic framework that enables computation of the deployment cost of a network (modeled using various spatial point processes) to answer the question posed by the paper's title. Then, the framework obtained is used along with a complexity model, which enables computing the information processing costs of a network, to compare the deployment cost of a cloud based network against that of a traditional LTE network, and to analyze why they are more economical. Using this framework and an exemplary budget, this paper shows that cloud-based radio access networks require approximately 10 to 15% less capital expenditure per square kilometer than traditional LTE networks. It also demonstrates that the cost savings depend largely on the costs of base stations and the mix of backhaul technologies used to connect base stations with data centers.

==> Cloud_RAN_System.tex <==
The analysis in this section relates costs induced by operating the communication infrastructure to costs required for processing information in a Cloud-\ac{RAN} system with a heterogeneous backhaul. This translation (or mapping) of costs is required to study the effect of information processing on the deployment cost of a network. The communication infrastructure spans multiple layers and is composed of the base station layer as well as the backhaul layer. Furthermore, the data center layer also processes all incoming and outgoing transmissions. The processing requires ample computational resources which are dependent directly on the parameterization and operating regime of the mobile network. %In order to evaluate these dependencies, we use the spatial point process model described in Section \ref{System_Model}. After which, Section \ref{Complexity_Model} presents a model that allows quantifying the data processing capabilities required (depending on the system parameters chosen).
A major contributor to the cost of a Cloud-\ac{RAN} system is the data center layer. If a data center is provided with too few computational resources, computational outage occurs. In which case, a transmission may not be successfully decoded though the channel quality is satisfactory. In contrast, if the system is over provisioned, it will be underutilized most of the time, which reduces the cost effectiveness of a centralized system.

  \begin{figure}[!h]
    \centering
\ifCLASSINFOpdf
  \includegraphics[width=7cm, height=7cm, keepaspectratio, viewport = 134 358 302 538]{protocol_stack.pdf}
\else
    \input{protocol.stack.tex}
\fi
    \caption{Protocol stack of a 3GPP LTE system and the functional split considered.}
    \label{fig:complexity_model:protocol_stack}
  \end{figure}

In general, the signal processing at a base station can be decomposed into an analog part and a digital baseband processing part. Usually, a Cloud-\ac{RAN} system centralizes only the digital processing while the analog processing remains at the base station. Furthermore, digital processing can be divided into a base station specific and a user specific part (see \cite{Doetsch.Doll.Mayer.etal.BellLabs.2013}). The base station specific part includes operations which need to be performed independent of the number of users or the actual amount of information transmitted by each user, e.g., Fast Fourier Transformation and resource de-mapping. In contrast, user specific processing covers all functions which scale with the number of users and the amount of information transmitted by them, e.g., forward error correction. In \cite{Wuebben.etal.SPM.2014}, various methods of separation between centralized and decentralized functionality have been discussed along with their impact on the backhaul capacity and latency required. In this paper, we consider a functional split above the detection stage and below the forward error correction stage as illustrated in Fig.~\ref{fig:complexity_model:protocol_stack}. In such cases, the backhaul capacity required scales linearly with the actual number of information bits encoded, i.e., either hard- or soft-detection in the uplink case. This allows exploiting the statistical multiplexing gain within the backhaul network which cannot be exploited if base station specific processing capabilities are centralized, e.g., as in the case of the \ac{CPRI}. The main challenge in implementing this functional split are the (portended) high backhaul latency and stringent real-time requirements of 3GPP LTE, e.g., of the \ac{HARQ} process (see \cite{Rost.Prasad.WCL.2014}).

In general, the processing requirements can be separated into those for uplink and downlink. As shown in \cite{Bhaumik.Chandrabose.Jataprolu.Kumar.Muralidhar.Polakos.Srinivasan.Woo.MobiCom.2012} based on the OpenAir platform (see \cite{OpenAir.2014} for details), the processing requirements in the uplink exceed those of the downlink by a factor of $5$ or more. A majority of the uplink processing resources are required for the decoder, i.e., more than $\unit[80]{\%}$ of the overall processing resources. Additionally, while the processing demand in the downlink is fairly predictable, it is highly variable in the uplink. The reason for which is a significant variation in the processing demand of a turbo decoder, which depends on the number of iterations and the information bits processed. In Section \ref{Complexity_Model}, we introduce an analytical model which predicts the processing demands of an uplink turbo-decoder. For the sake of brevity and due to the dominance of the uplink decoder processing requirements over the others, this paper considers solely the uplink decoder for dimensioning the data processing resources required. 



==> Cloud_RAN_System_v1.tex <==
The analysis in this section relates costs induced by operating the communication infrastructure to costs required for processing information in a Cloud-\ac{RAN} system with a heterogeneous backhaul. The communication infrastructure spans multiple layers and is composed of the base station layer as well as the backhaul layer. Furthermore, the data center layer processes all incoming and outgoing transmissions. The processing requires ample computational resources which are dependent directly on the parameterization and operating regime of the mobile network. In order to evaluate these dependencies, we use the spatial point process model described in Section \ref{System_Model}. After which, Section \ref{Complexity_Model} presents a model that allows quantifying the data processing capabilities required (depending on the system parameters chosen).

A major contributor to the cost of a Cloud-\ac{RAN} system is the data center layer. Dimensioning individual data centers is a critical task. If a data center is provided with too few computational resources, computational outage occurs. In this case, a transmission may not be successfully decoded though the channel quality is satisfactory. In contrast, if the system is over provisioned, it will be underutilized most of the time, which reduces the cost effectiveness of a centralized system.

\ifCLASSINFOpdf
\else
  \begin{figure}[!h]
    \centering
    \input{protocol.stack.tex}
    \caption{Protocol stack of a 3GPP LTE system and considered functional split}
    \label{fig:complexity_model:protocol_stack}
  \end{figure}
\fi

In general, the signal processing at a base station can be decomposed into an analog part and a digital baseband processing part. Usually, a Cloud-\ac{RAN} system centralizes only the digital processing while the analog processing remains at the base station. Furthermore, digital processing can be divided into a base station specific and a user specific part (see \cite{Doetsch.Doll.Mayer.etal.BellLabs.2013}). The base station specific part includes operations which need to be performed independent of the number of users or the actual amount of information transmitted by each user, e.g., Fast Fourier Transformation and resource de-mapping. In contrast, user specific processing covers all functions which scale with the number of users and the amount of information transmitted by them, e.g., forward error correction. In \cite{Wuebben.etal.SPM.2014}, various methods of separation between centralized and decentralized functionality have been discussed along with their impact on the backhaul capacity and latency required. In this paper, we consider a functional split above the detection stage and below the forward error correction stage as illustrated in Fig.~\ref{fig:complexity_model:protocol_stack}. In such cases, the backhaul capacity required scales linearly with the actual number of information bits encoded, i.e., either hard- or soft-detection in the uplink case. This allows exploiting the statistical multiplexing gain within the backhaul network which cannot be exploited if base station specific processing capabilities are centralized, e.g., as in the case of the \ac{CPRI}. The main challenge in implementing this functional split are the (portended) high backhaul latency and stringent real-time requirements of 3GPP LTE, e.g., of the \ac{HARQ} process (see \cite{Rost.Prasad.WCL.2014}).

In general, the processing requirements can be separated into those for uplink and downlink. As shown in \cite{Bhaumik.Chandrabose.Jataprolu.Kumar.Muralidhar.Polakos.Srinivasan.Woo.MobiCom.2012} based on the OpenAir platform (see \cite{OpenAir.2014} for details), the processing requirements in the uplink exceed those of the downlink by a factor of $5$ or more. A majority of the uplink processing resources are required for the decoder, i.e., more than $\unit[80]{\%}$ of the overall processing resources. Additionally, while the processing demand in the downlink is fairly predictable, it is highly variable in the uplink. The reason for which is a significant variation in the processing demand of a turbo decoder, which depends on the number of iterations and the information bits processed. In Section \ref{Complexity_Model}, we introduce an analytical model which predicts the processing demands of an uplink turbo-decoder. For the sake of brevity and due to the dominance of the uplink decoder processing requirements over the others, this paper considers solely the uplink decoder for dimensioning the data processing resources required. 



==> Complexity_Model.tex <==
  \begin{figure}
    \centering
\ifCLASSINFOpdf
  \includegraphics[width=10cm, height=10cm, keepaspectratio, viewport = 132 342 473 526]{Complexity_SNR_theory.pdf}
\else
    \input{Complexity_SNR_theory.tex}
\fi
    \caption{A comparison of theoretical and actual LTE decoder complexity.}
    \label{fig:complexity_model:complexity_over_snr}
  \end{figure}
The uplink processing complexity is determined by the turbo decoder. Let $\gamma$ denote the channel's instantaneous \ac{SNR} and $k$ denote the index of the chosen \ac{MCS}. Then, the complexity of the decoding process scales both with the number of information bits $I(\gamma, k)$ processed and the number of iterations $L(\gamma, k)$ required to decode a transport block of duration $t_s$ and bandwidth $B_s$. In the following, we use the normalized data processing requirement $\mathcal{D}_\text{norm}(\gamma, k) = I(\gamma, k)L(\gamma, k)/(t_s B_s)$ to quantify the required data processing resources which are measured in bit-iterations per channel use (pcu). The advantage of this approach is its independence of frame format and bandwidth (similar to spectral efficiency).

In contrast, Bhaumik et al. (in \cite{Bhaumik.Chandrabose.Jataprolu.Kumar.Muralidhar.Polakos.Srinivasan.Woo.MobiCom.2012}) performed a quantitative assessment of the required processing \emph{time} in an uplink LTE system, i.e., for a specific \ac{MCS} $k$, the time required to process one transport block has been determined. Although this empirical study is very important and valuable, it does not allow for generalized inferences about the stochastic behavior of the uplink decoding process as well as the centralization gain in a Cloud-\ac{RAN} system. In \cite{Rost.Talarico.Valenti.TWC.2014}, the authors derive an analytical model which allows evaluating the data processing requirements of a set of $N_\text{cloud}$ base stations. Fig. \ref{fig:complexity_model:complexity_over_snr} (taken from \cite{Rost.Talarico.Valenti.TWC.2014}) shows a comparison of empirical measurements and the analytical model. It is apparent that complexity clearly varies with the \ac{SNR}. In fact, if the data rate $R_k$ of a chosen \ac{MCS} $k$ is close to capacity, the processing resources required also increase super-linearly. In order to evaluate the extent of this dependence, we introduce the model derived in \cite{Rost.Talarico.Valenti.TWC.2014} briefly and use it to quantify the data processing resources required in a Cloud-\ac{RAN} system.

The data processing resources required depend on the following parameters which originate
from the decoder power consumption model in \cite{Grover.Woyach.Sahai.JSAC.2011} ( and is applied in \cite{Rost.Talarico.Valenti.TWC.2014}). The first parameter chosen is the \ac{MCS} $k$ which determines the code rate $R_k$ at which the system is operated. Then, we consider a target channel outage probability $\hat\epsilon_\text{channel}$ and a complexity scaling function $K(\hat\epsilon_\text{channel})$. The decoder connectivity $\zeta$ models the connectivity of the message passing algorithm considered in \cite{Grover.Woyach.Sahai.JSAC.2011}. Based on an empirical study, \cite{Rost.Talarico.Valenti.TWC.2014} details a suitable parameterization for a 3GPP LTE decoder whose parameters are $\zeta = 4$ and $K(0.1) = 0.15$ (with the assumption $\hat\epsilon_\text{channel} = 0.1$). Based on this model, \cite{Rost.Talarico.Valenti.TWC.2014} shows that the complexity of the decoder is well approximated by
\begin{equation}
  \mathcal{D}_\text{norm}(\gamma, k) = \frac{R_k}{\log_2\left(\zeta - 1\right)}\left(\log_2\left(\frac{\zeta - 2}{K(\hat\epsilon_\text{channel})\zeta}\right) - 2\log_2\left(\log_2(1 + \gamma) - R_k\right) \right).
  \label{eq:complexity.model:100}
\end{equation}
Another critical system parameterization is the link-adaptation, which determines the minimum required \ac{SNR} at which a specific \ac{MCS} $k$ is chosen. Ideally, if perfect random codes of infinite length are assumed, we can use the \ac{SNR} thresholds $\gamma_{c, k} = 2^{R_k} - 1$, which denote the threshold in the Shannon capacity case for rate $R_k$. However, a practical system will not operate at capacity and the \ac{SNR} thresholds of a decoder (that is deployed in practice) are given by $\gamma_{r, k} =\gamma_{r, \text{offset}} \,\gamma_{c, k}$ where $\gamma_{r, \text{offset}}$ determines the quality of the decoder. The smaller the value of $\gamma_{r, \text{offset}}$, closer the system operates to capacity but greater the number of iterations necessary to decode a codeword. On the other hand, if the offset is higher, fewer processing resources are required which implies an inherent trade-off between processing resources provided (and their associated costs) and the performance delivered.

  \begin{figure}[!h]
    \centering
\ifCLASSINFOpdf
    \subfigure[Outage processing resources per base station]{\includegraphics[width=7cm, height=7cm, keepaspectratio, viewport = 131 348 360 526]{Complexity_outage_network_Nusers_with_pl.pdf}}
    \subfigure[Processing demand in number of servers]{\includegraphics[width=7cm, height=7cm, keepaspectratio, viewport = 132 348 360 526]{Complexity_outage_network_Nusers_with_pl_units.pdf}}
\else
    \subfigure[Outage processing resources per base station]{\input{Complexity_outage_network_Nusers_with_pl.tex}}
    \subfigure[Processing demand in number of servers]{\input{Complexity_outage_network_Nusers_with_pl_units.tex}}
\fi
    \caption{Data processing capabilities required to ensure per-base-station computational outage probability $\hat\epsilon_\text{comp}$. The dashed lines denote the equivalent processing power required in a distributed deployment without exploiting computational gain.}
    \label{fig:complexity_model:complexity_network}
  \end{figure}
Based on this model, \cite{Rost.Talarico.Valenti.TWC.2014} derives expressions for the mean $\Exp\left[\mathcal{D}(\gamma, k)\right]$ and the variance $\text{Var}\left[\mathcal{D}(\gamma, k)\right]$ of the processing resources. Other critical system parameters are the processing outage probability $\epsilon_\text{comp}(N_\text{cloud})$ and the outage processing demand $\mathcal{D}_\text{outage}(\hat\epsilon_\text{comp}, N_\text{cloud})$, which are related by
\begin{equation}
   \epsilon_\text{comp}(N_\text{cloud}) = \Prob\left[
       \sum_{i=1}^{N_\text{cloud}} \mathcal{D}_\text{norm}(\gamma_i | k) > \mathcal{D}_\text{outage}(\hat\epsilon_\text{comp}, N_\text{cloud})
   \right] 
  \label{eq:complexity.model:120}
\end{equation}
Here, $\mathcal{D}_\text{outage}(\hat\epsilon_\text{comp}, N_\text{cloud})$ quantifies the normalized data processing resources required in order to guarantee a maximum per-base-station computational outage probability $\hat\epsilon_\text{comp} = 0.1$. Fig. \ref{fig:complexity_model:complexity_network}(a) shows the normalized outage processing resources as a function of the number of centralized base stations $N_\text{cloud}$ and the decoder quality characterized by $\gamma_{r, \text{offset}}$.

Using Fig. \ref{fig:complexity_model:complexity_network}(a), we can estimate the required number of CPU cores. We consider a 3GPP LTE system with $\unit[10]{MHz}$ channel bandwidth where one user may occupy at most $45$ physical resource blocks, each consisting of $12\times 7$ sub-carriers in a sub-frame of $t_s = \unit[0.5]{ms}$ duration. Therefore, the data processing resources required are given by $\mathcal{D}_\text{abs} = \mathcal{D}_\text{outage} \times 45 \times 12 \times 7/\unit[0.5]{ms} \approx \mathcal{D}_\text{outage} \times 7.5 \times 10^6 \, \nicefrac{cu}{s}$. A typical turbo-decoder implementation requires up to $1,000$ \acp{FLOP} per bit-iteration (see \cite{Valenti.Sun.IJWIN.2001}), i.e., the data processing demand required can be determined by $\mathcal{D}_\text{outage} \times 7.5 \, \nicefrac{\text{GFLOP}}{\text{bit-iter}\cdot\text{s}}$. Please note that $\mathcal{D}_\text{outage}$ determines the bit-iterations per channel use required. As a reference, the Intel Xeon 4870 is a 10 core processor which achieves $96 \, \nicefrac{\text{GFLOP}}{\text{s}}$ and is typically packaged on a quad socket board. Such a server setup (including 128 GB RAM) would cost about \$ 40,000. If $\mathcal{D}_\text{unit}$ is the data processing demand in number of such server setups, then Fig.  \ref{fig:complexity_model:complexity_network}(b) shows the processing power required to operate a Cloud-\ac{RAN} system \textcolor{red}{The relationship between $\mathcal{D}_\text{abs}$ and $\mathcal{D}_\text{unit}$ is not mentioned. Without this connection, it seems rather arbitrary to define them.}. These values will be used in Section \ref{Obtaining_Cost_Values}  and Section \ref{Numerical_Evaluation} as inputs to enable us to compute the deployment cost of the network.


==> Complexity_gain_Nusers.tex <==
\begingroup
\unitlength=1mm
\psset{xunit=1.30000mm, yunit=14.28163mm, linewidth=0.1mm}
\psset{arrowsize=2pt 3, arrowlength=1.4, arrowinset=.4}\psset{axesstyle=frame}
\begin{pspicture}(-11.53846, -0.12032)(50.00000, 4.50100)
\rput(-1.53846, -0.35010){%
\psaxes[subticks=0, labels=all, xsubticks=1, ysubticks=1, Ox=0, Oy=1, Dx=10, Dy=0.5]{-}(0.00000, 1.00000)(0.00000, 1.00000)(50.00000, 4.50100)%
\multips(10.00000, 1.00000)(10.00000, 0.0){4}{\psline[linecolor=black, linestyle=dotted, linewidth=0.2mm](0, 0)(0, 3.50100)}
\multips(0.00000, 1.50000)(0, 0.50000){6}{\psline[linecolor=black, linestyle=dotted, linewidth=0.2mm](0, 0)(50.00000, 0)}
\rput[b](25.00000, 0.22978){Number of users $N_\text{cloud}$}
\rput[t]{90}(-10.00000, 2.75050){{$g_\text{comp}$}}
\psclip{\psframe(0.00000, 1.00000)(50.00000, 4.50100)}
\psline[linecolor=blue, plotstyle=curve, linewidth=0.4mm, showpoints=true, linestyle=solid, linecolor=blue, dotstyle=o, dotscale=1.2 1.2, linewidth=0.4mm](1.00000, 1.00000)(2.00000, 1.44582)(3.00000, 1.65360)(4.00000, 1.79903)(5.00000, 1.90852)(10.00000, 2.21682)(20.00000, 2.46026)(30.00000, 2.57008)(50.00000, 2.67715)
\psline[linecolor=red, plotstyle=curve, linewidth=0.4mm, showpoints=true, linestyle=solid, linecolor=red, dotstyle=triangle, dotscale=1.2 1.2, linewidth=0.4mm](1.00000, 1.00000)(2.00000, 1.42001)(3.00000, 1.61196)(4.00000, 1.74461)(5.00000, 1.84357)(10.00000, 2.11813)(20.00000, 2.33074)(30.00000, 2.42549)(50.00000, 2.51715)
\psline[linecolor=black, plotstyle=curve, linewidth=0.4mm, showpoints=true, linestyle=solid, linecolor=black, dotstyle=diamond, dotscale=1.2 1.2, linewidth=0.4mm](1.00000, 1.00000)(2.00000, 1.37265)(3.00000, 1.54685)(4.00000, 1.66575)(5.00000, 1.75369)(10.00000, 1.99428)(20.00000, 2.17724)(30.00000, 2.25784)(50.00000, 2.33530)
\endpsclip
\psframe[linecolor=black, fillstyle=solid, fillcolor=white, shadowcolor=lightgray, shadowsize=1mm, shadow=true](3.84615, 3.66076)(29.23077, 4.57102)
\rput[l](10.76923, 4.36096){\footnotesize{$\gamma_\text{r, offset}=\unit[0.2]{dB}$}}
\psline[linecolor=blue, linestyle=solid, linewidth=0.3mm](5.38462, 4.36096)(8.46154, 4.36096)
\psline[linecolor=blue, linestyle=solid, linewidth=0.3mm](5.38462, 4.36096)(8.46154, 4.36096)
\psdots[linecolor=blue, linestyle=solid, linewidth=0.3mm, dotstyle=o, dotscale=1.2 1.2, linecolor=blue](6.92308, 4.36096)
\rput[l](10.76923, 4.11589){\footnotesize{$\gamma_\text{r, offset}=\unit[0.5]{dB}$}}
\psline[linecolor=red, linestyle=solid, linewidth=0.3mm](5.38462, 4.11589)(8.46154, 4.11589)
\psline[linecolor=red, linestyle=solid, linewidth=0.3mm](5.38462, 4.11589)(8.46154, 4.11589)
\psdots[linecolor=red, linestyle=solid, linewidth=0.3mm, dotstyle=triangle, dotscale=1.2 1.2, linecolor=red](6.92308, 4.11589)
\rput[l](10.76923, 3.87082){\footnotesize{$\gamma_\text{r, offset}=\unit[1]{dB}$}}
\psline[linecolor=black, linestyle=solid, linewidth=0.3mm](5.38462, 3.87082)(8.46154, 3.87082)
\psline[linecolor=black, linestyle=solid, linewidth=0.3mm](5.38462, 3.87082)(8.46154, 3.87082)
\psdots[linecolor=black, linestyle=solid, linewidth=0.3mm, dotstyle=diamond, dotscale=1.2 1.2, linecolor=black](6.92308, 3.87082)
}\end{pspicture}
\endgroup
\endinput


==> backup.tex <==
The analysis in this work relates costs induced by operating the communication infrastructure to costs required for information processing
in a Cloud-\ac{RAN} system with heterogeneous backhaul. The communication infrastructure covers multiple layers composed of small-cells and macro-cells as well as
the connecting heterogeneous backhaul layer. On top, a data-center layer processes all incoming and outgoing transmissions. This processing requires sufficient computational resources which
dependent directly on the parameterization and operating regime of the mobile network. In order to evaluate these dependencies, we first describe in
Section \ref{System_Model} a spatial point process model which is used to model the multi-layer mobile network and its connecting infrastructure. Afterwards,
Section \ref{Complexity_Model} presents a model which allows for quantifying the required data processing capabilities depending on the chosen system parameters.

A major contributor to the costs of a Cloud-\ac{RAN} system is the data-center layer.
Dimensioning each data-center is a critical task. If a data-center is provided with two few computational resources, computational outage occurs. In this case,
a transmission may not be successfully decoded although the channel is of sufficient quality. By contrast, if the system is over-provisioned, it will be under-utilized
for most of the time which would reduce the actual cost-benefits of a centralized system.

\ifCLASSINFOpdf
\else
  \begin{figure}
    \centering
    \input{protocol.stack.tex}
    \caption{Protocol stack of a 3GPP LTE system and considered functional split}
    \label{fig:complexity_model:protocol_stack}
  \end{figure}
\fi
In general, the signal processing at a base station can be decomposed into an analog part and a digital baseband processing part. Usually, a Cloud-\ac{RAN} system
centralizes only the digital processing while the analog processing remains at the base station. Furthermore, the digital processing can be divided into a 
cell-specific and a user-specific part \cite{Doetsch.Doll.Mayer.etal.BellLabs.2013}. The cell-specific part includes operations which need to be performed independent of the
number of users or the actual amount of information bits transmitted by each user, e.\,g. Fast Fourier Transformation and resource demapping.
By contrast, the user-specific processing covers all functions which scale with the number of users and their transmitted information bits, e.\,g. forward error correction.
In \cite{Wuebben.etal.SPM.2014}, different splits between centralized and decentralized functionality have been discussed as well as their impact on the required backhaul capacity and latency.

In this paper, we consider a functional split above the detection and below the forward error correction as illustrated in Fig. \ref{fig:complexity_model:protocol_stack}.
In case of this split, the required backhaul capacity scales linearly with the actual encoded information bits, either hard detected or soft detected in the case of
uplink. This allows for exploiting the statistical multiplexing gain within the backhaul network which cannot be exploited if per-cell processing capabilities
are centralized, e.\,g. in the case of the \ac{CPRI}. The main challenge to implement this functional split is the potentially high backhaul latency and the hard real-time
requirements of 3GPP LTE, e.\,g. of the \ac{HARQ} process \cite{Rost.Prasad.WCL.2014}.

In general, the processing requirements can be separated into those for uplink and those for downlink. As shown in \cite{Bhaumik.Chandrabose.Jataprolu.Kumar.Muralidhar.Polakos.Srinivasan.Woo.MobiCom.2012} based on the OpenAir platform \cite{OpenAir.2014},
the processing requirements in uplink exceed those for downlink by a factor of $5$ and more. 
The main part of uplink processing resources is required for the decoder, i.\,e. more than $\unit[80]{\%}$ of the overall processing resources. 
In addition, while the processing demand in downlink
is fairly predictable, it is highly random in the uplink. The reason is the strong variation of processing demand of a turbo-decoder which depends on the number of
iterations and processed information bits. 
In Section \ref{Complexity_Model}, we introduce an analytical model which is able to predict the processing demands of an uplink turbo-decoder.
Due to the domination of processing requirements by the uplink decoder as well as for the sake of brevity, 
we consider in this paper only the uplink decoder for the dimensioning the required data processing resources. 


